Sketch2Mesh: Reconstructing and Editing 3D Shapes from Sketches

Reconstructing 3D shape from 2D sketches has long been an open problem because the sketches only provide very sparse and ambiguous information. In this paper, we use an encoder/decoder architecture for the sketch to mesh translation. When integrated into a user interface that provides camera parameters for the sketches, this enables us to leverage its latent parametrization to represent and refine a 3D mesh so that its projections match the external contours outlined in the sketch. We will show that this approach is easy to deploy, robust to style changes, and effective. Furthermore, it can be used for shape refinement given only single pen strokes. We compare our approach to state-of-the-art methods on sketches -- both hand-drawn and synthesized -- and demonstrate that we outperform them.

==> figs/editing.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{figure*}
\begin{center}
 %\includegraphics[width=.45\textwidth]{figs/robustness.pdf}
 %,grid,tics=5
 	\begin{overpic}[clip, trim=0cm 7.0cm 0cm 0cm,width= .95\textwidth]{figs/editing.pdf}
 
 	
 	\put(5,36){\small{input}}
 	\put(18,36){\small{reconstruction}}
 	
 	\put(33,36){\small{silhouette gap}}
 	\put(49,36){\small{silhouette refinement}}
 	
 	\put(69,36){\small{contour gap}}
 	\put(85,36){\small{contour refinement}}
 	
 \end{overpic}
\end{center}
\vspace{-3mm}
   \caption{\textbf{Local editing.}. }
\label{fig:robustness}
\end{figure*}

==> figs/fb_prediction.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{figure}
\begin{center}
\begin{tabular}{ccc}
 \includegraphics[width=.13\textwidth]{figs/mask_input.png}&
 \includegraphics[width=.13\textwidth]{figs/mask_gt.png} &
 \includegraphics[width=.13\textwidth]{figs/mask_pred.png} \\
    (a) & (b) & (c)
\end{tabular}
\end{center}
\vspace{-3mm}
   \caption{\textbf{Foregroud/background mask prediction} is prone to errors drawing style changes: \textbf{(a)} input synthetic sketch, from \textit{SketchFD}'s style, \textbf{(b)} ground truth mask, \textbf{(c)} prediction by the network trained on \textit{DeCarlo}'s style.}
\label{fig:fb_prediction}
\end{figure}

==> tables/cars_sketchDR.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{table*}[ht]
    \caption{\textbf{Single view reconstruction results on ShapeNet/Cars.} Blabla look at out metrics blabla.}
	\label{tab:cars_sketchDR}
	\begin{center}
		\scalebox{0.65}{
			\begin{tabular}{c|c|c| c | c}
				\Xhline{2\arrayrulewidth}
				Metric & Method & SketchDR & DeCarlo & Our \\
				\Xhline{2\arrayrulewidth}
				\multirow{10}{*}{CD-$l_2 \cdot 10^3$ $\downarrow$}
                &Pix2Vox~\cite{Groueix18a}&2.710&3.529&3.146\\
                &DISN~\cite{Groueix18a}&7.754&4.566&11.594\\
                &DISN (silhouette)~\cite{Groueix18a}&1.708
&3.601&2.246\\
				\cline{2-5}
				&MeshSDF  &1.815&3.227&\\
				&MeshSDF (silhouette) &1.515&2.454&\\
				&MeshSDF (chamfer) &1.516&2.761&\\
				\cline{2-5}
				&AtlasNet ~\cite{Groueix18a}&&&\\
				&AtlasNet (silhouette)~\cite{Groueix18a}&&&\\
				&AtlasNet (chamfer)~\cite{Groueix18a}&&&\\
				\Xhline{2\arrayrulewidth}
				
				\multirow{10}{*}{Normal Consistency $\uparrow$}&Pix2Vox~\cite{Groueix18a}&0.8921&0.8711&0.8627\\
                &DISN~\cite{Groueix18a}&0.7584&0.7966&0.6936\\
                &DISN (silhouette)~\cite{Groueix18a}&0.9089&0.8877
&0.8979\\
				\cline{2-5}
				&MeshSDF  &0.9094&0.8967&\\
				&MeshSDF (silhouette) &0.9234&0.9117&\\
				&MeshSDF (chamfer) &0.9209&0.9113&\\
				\cline{2-5}
				&AtlasNet ~\cite{Groueix18a}&&&\\
				&AtlasNet (silhouette)~\cite{Groueix18a}&&&\\
				&AtlasNet (chamfer)~\cite{Groueix18a}&&&\\
				\Xhline{2\arrayrulewidth}
		\end{tabular}}
	\end{center}
\end{table*}

==> tables/refinement_cars.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

\begin{table}[ht]
    \caption{\textbf{Refinement on cars sketches.}
		Reconstruction metrics for encoder/decoder architectures trained on Suggestive synthetic sketches of cars, and tested on all 3 datasets. We show results without refinement (\textit{raw}), with differentiable rasterization based refinement ($\mathcal{L}_{F/B}$), and based on matching external contours ($\mathcal{L}_{CD}$).
		}
	\label{tab:refinement_cars}
	\begin{center}
		\scalebox{0.65}{
			\begin{tabular}{c|c|c|c|c}
				%\Xhline{2\arrayrulewidth}
				%Metric & Method & SketchDR & DeCarlo & Human \\
				%\Xhline{2\arrayrulewidth}
				\Xhline{2\arrayrulewidth}
				Metric & Method & \multicolumn{3}{c}{Test Drawing Style} \\
				\cline{3-5}
				&  & DeCarlo& SketchFD  & HumanCars \\
				\Xhline{2\arrayrulewidth}
				\multirow{6}{*}{CD-$l_2 \cdot 10^3$ $\downarrow$}
				&MeshSDF \textit{raw}         &1.613&4.658&6.818\\
				&MeshSDF + $\mathcal{L}_{F/B}$&1.400&4.253&5.752\\
				&MeshSDF + $\mathcal{L}_{CD}$ &1.420&3.132&4.395\\
				\cline{2-5}
				&AtlasNet \textit{raw}         &1.532&3.552&4.592\\
				&AtlasNet + $\mathcal{L}_{F/B}$&\textbf{1.333}&2.721&3.143\\
				&AtlasNet + $\mathcal{L}_{CD}$ &1.500&\textbf{2.371}&\textbf{2.927}\\
				\Xhline{2\arrayrulewidth}
				
				\multirow{6}{*}{Normal Consistency $\uparrow$}
				&MeshSDF \textit{raw}         &91.14&84.73&81.40\\
				&MeshSDF + $\mathcal{L}_{F/B}$&\textbf{92.41}&86.18&83.88\\
				&MeshSDF + $\mathcal{L}_{CD}$ &92.20&\textbf{87.00}&\textbf{84.75}\\
				\cline{2-5}
				&AtlasNet \textit{raw}         &87.63&83.46&81.50\\
				&AtlasNet + $\mathcal{L}_{F/B}$&88.12&84.41&83.32\\
				&AtlasNet + $\mathcal{L}_{CD}$ &87.88&84.88&83.14\\
				\Xhline{2\arrayrulewidth}
		\end{tabular}}
	\end{center}
\end{table}

\comment{	\begin{center}
		\scalebox{0.65}{
			\begin{tabular}{c|c|c|c|c}
				%\Xhline{2\arrayrulewidth}
				%Metric & Method & SketchDR & DeCarlo & Human \\
				%\Xhline{2\arrayrulewidth}
				\Xhline{2\arrayrulewidth}
				Metric & Method & \multicolumn{3}{c}{Test Drawing Style} \\
				\cline{3-5}
				&  & DeCarlo& SketchFD  & HumanCars \\
				\Xhline{2\arrayrulewidth}
				\multirow{6}{*}{CD-$l_2 \cdot 10^3$ $\downarrow$}
				&MeshSDF \textit{raw}         &1.815&3.231&2.534\\
				&MeshSDF + $\mathcal{L}_{F/B}$&1.515&2.538&2.054\\
				&MeshSDF + $\mathcal{L}_{CD}$ &1.516&2.419&2.047\\
				\cline{2-5}
				&AtlasNet \textit{raw}         &1.636&2.386&2.057\\
				&AtlasNet + $\mathcal{L}_{F/B}$&\textbf{1.407}&\textbf{2.167}&\textbf{1.621}\\
				&AtlasNet + $\mathcal{L}_{CD}$ &1.487&2.205&1.802\\
				\Xhline{2\arrayrulewidth}
				
				\multirow{6}{*}{Normal Consistency $\uparrow$}
				&MeshSDF \textit{raw}         &90.94&89.67&89.06\\
				&MeshSDF + $\mathcal{L}_{F/B}$&\textbf{92.34}&90.92&91.02\\
				&MeshSDF + $\mathcal{L}_{CD}$ &92.09&\textbf{91.23}&\textbf{91.03}\\
				\cline{2-5}
				&AtlasNet \textit{raw}         &87.62&87.28&85.95\\
				&AtlasNet + $\mathcal{L}_{F/B}$&88.22&87.46&86.75\\
				&AtlasNet + $\mathcal{L}_{CD}$ &87.94&87.51&86.58\\
				\Xhline{2\arrayrulewidth}
		\end{tabular}}
\end{center}}

==> tables/refinement_chairs.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US
\begin{table}[ht]
	\caption{\textbf{Refinement on chairs sketches.}
		Reconstruction metrics for encoder/decoder architectures trained on Suggestive synthetic sketches of chairs, and tested on all 3 datasets. Note that ProSketch are drawn using a different focal length than our training data, making generalization even more challenging for our networks. We show results without refinement (\textit{raw}), with differentiable rasterization based refinement ($\mathcal{L}_{F/B}$), and based on matching external contours ($\mathcal{L}_{CD}$).
		\BG{Can't we merge this table and Tab. \ref{tab:refinement_cars}? the captions are almost identical and could be factored?}
	}
	\label{tab:refinement_chairs}

\end{table}
\comment{
\begin{table}[ht]
    \caption{\textbf{Refinement on ShapeNet/Chairs.} Blabla look at out metrics blabla. \BG{Again here on AtlasNet silh looks better than chamfer.}}
	\label{tab:refinement_chairs}
	\begin{center}
		\scalebox{0.65}{
			\begin{tabular}{c|c|c| c }
				\Xhline{2\arrayrulewidth}
				Metric & Method & SketchDR & DeCarlo \\
				\Xhline{2\arrayrulewidth}
				\multirow{6}{*}{CD-$l_2 \cdot 10^3$ $\downarrow$}
				&MeshSDF  &7.770&12.290\\
				&MeshSDF (silhouette) &6.517&10.761\\
				&MeshSDF (chamfer) &6.737&9.524\\
				\cline{2-4}
				&AtlasNet~\cite{Groueix18a}&6.066&8.361\\
				&AtlasNet (silhouette)~\cite{Groueix18a}&5.186&7.094\\
				&AtlasNet (chamfer)~\cite{Groueix18a}&5.409&7.544\\
				\Xhline{2\arrayrulewidth}
				
				\multirow{5}{*}{Normal Consistency $\uparrow$}
				&MeshSDF  &80.49&76.76\\
				&MeshSDF (silhouette) &84.43&80.39\\
				&MeshSDF (chamfer) &83.10&81.00\\
				\cline{2-4}
				&AtlasNet~\cite{Groueix18a}&77.27&74.06\\
				&AtlasNet (silhouette)~\cite{Groueix18a}&78.84&76.11\\
				&AtlasNet (chamfer)~\cite{Groueix18a}&78.03&75.41\\
				\Xhline{2\arrayrulewidth}
		\end{tabular}}
	\end{center}
\end{table}}
